Efficient high-order singular quadrature schemes in magnetic fusion

Several problems in magnetically confined fusion, such as the computation of exterior vacuum fields or the decomposition of the total magnetic field into separate contributions from the plasma and the external sources, are best formulated in terms of integral equation expressions. Based on Biot-Savart-like formulae, these integrals contain singular integrands. The regularization method commonly used to address the computation of various singular surface integrals along general toroidal surfaces is low-order accurate, and therefore requires a dense computational mesh in order to obtain sufficient accuracy. In this work, we present a fast, high-order quadrature scheme for the efficient computation of these integrals. Several numerical examples are provided demonstrating the computational efficiency and the high-order accurate convergence. A corresponding code for use in the community has been publicly released.

==> figs/quadrature/polar-interp-source.tex <==
\begin{tikzpicture}[scale=7] %<<<

  \newcommand*\spherex[2]{(sin(#1)*sin(#2))}
  \newcommand*\spherey[2]{(sin(#1)*cos(#2)*cos(15)+sin(15)*cos(#1))}
  \newcommand*\spherez[2]{(cos(#1)*cos(15)+sin(15)*sin(#1)*cos(#2))}

  \newcommand*{\PLat}{60}%{90}
  \newcommand*{\PLon}{35}%{0}
  \newcommand*{\dLat}{12}%
  \newcommand*{\dLon}{8}%
  \newcommand*{\XX}[2]{(sin(#2)*0.5*(0.5+0.5*cos(#1)))}
  \newcommand*{\YY}[2]{(cos(#2)*0.5*(0.5+0.5*cos(#1)))}

  \newcommand*\drawpatch[3]{ %<<<
    \foreach \y in {-0.5,-0.45,...,0.55} {
      \foreach \x in {-0.5,-0.45,...,0.5} {
        \draw[black!100] ({\spherex{#1+\x*#3}{#2+\y*#3}},{\spherez{#1+\x*#3}{#2+\y*#3}}) --  ({\spherex{#1+(\x+0.05)*#3}{#2+\y*#3}},{\spherez{#1+(\x+0.05)*#3}{#2+\y*#3}}) ;
        \draw[black!100] ({\spherex{#1+\y*#3}{#2+\x*#3}},{\spherez{#1+\y*#3}{#2+\x*#3}}) --  ({\spherex{#1+\y*#3}{#2+(\x+0.05)*#3}},{\spherez{#1+\y*#3}{#2+(\x+0.05)*#3}}) ;
      }
    }

    \foreach \p in {10,30,...,370} {
      \foreach \t in {20,25,...,180} {
        \draw[red!100,line width=0.15mm] ({\spherex{#1+\XX{\t}{\p}*#3}{#2+\YY{\t}{\p}*#3}},{\spherez{#1+\XX{\t}{\p}*#3}{#2+\YY{\t}{\p}*#3}}) --  ({\spherex{#1+(\XX{(\t+5.00)}{\p})*#3}{#2+\YY{(\t+5.00)}{\p}*#3}},{\spherez{#1+(\XX{(\t+5.00)}{\p})*#3}{#2+\YY{(\t+5.00)}{\p}*#3}}) ;
      }
    }
    \foreach \p in {10,15,...,370} {
      \foreach \t in {20,40,...,180} {
        \draw[red!100,line width=0.15mm] ({\spherex{#1+\XX{\t}{\p}*#3}{#2+\YY{\t}{\p}*#3}},{\spherez{#1+\XX{\t}{\p}*#3}{#2+\YY{\t}{\p}*#3}}) --  ({\spherex{#1+(\XX{(\t)}{\p+5.00})*#3}{#2+\YY{(\t)}{\p+5.00}*#3}},{\spherez{#1+(\XX{(\t)}{\p+5.00})*#3}{#2+\YY{(\t)}{\p+5.00}*#3}}) ;
      }
    }
    \draw[red,fill=red] ({\spherex{#1+\XX{20}{130}*#3}{#2+\YY{20}{130}*#3}},{\spherez{#1+\XX{20}{130}*#3}{#2+\YY{20}{130}*#3}}) circle [radius=0.2pt];

    \foreach \y in {0.25,0.30,...,0.55} {
      \foreach \x in {-0.45,-0.40,...,-0.20} {
        \draw[black!100,line width=0.2mm] ({\spherex{#1+\y*#3}{#2+\x*#3}},{\spherez{#1+\y*#3}{#2+\x*#3}}) --  ({\spherex{#1+\y*#3}{#2+(\x+0.05)*#3}},{\spherez{#1+\y*#3}{#2+(\x+0.05)*#3}}) ;
      }
    }
    \foreach \y in {0.25,0.30,...,0.5} {
      \foreach \x in {-0.45,-0.40,...,-0.15} {
        \draw[black!100,line width=0.2mm] ({\spherex{#1+\y*#3}{#2+\x*#3}},{\spherez{#1+\y*#3}{#2+\x*#3}}) --  ({\spherex{#1+(\y+0.05)*#3}{#2+\x*#3}},{\spherez{#1+(\y+0.05)*#3}{#2+\x*#3}}) ;
      }
    }
    \foreach \y in {0.25,0.30,...,0.55} {
      \foreach \x in {-0.45,-0.40,...,-0.15} {
        \draw[black,fill=black] ({\spherex{#1+\y*#3}{#2+\x*#3}},{\spherez{#1+\y*#3}{#2+\x*#3}}) circle [radius=0.2pt];
      }
    }

    \draw[blue,fill=blue] ({\spherex{#1}{#2}},{\spherez{#1}{#2}}) circle [radius=0.3pt];

    \node (A) at ({\spherex{#1-0.50*#3}{#2-0.60*#3}},{\spherez{#1-0.50*#3}{#2-0.60*#3}}) {};
    \node (B) at ({\spherex{#1+0.50*#3}{#2-0.55*#3}},{\spherez{#1+0.50*#3}{#2-0.55*#3}}) {};
    \node (C) at ({\spherex{#1+0.55*#3}{#2-0.50*#3}},{\spherez{#1+0.55*#3}{#2-0.50*#3}}) {};
    \node (D) at ({\spherex{#1+0.55*#3}{#2+0.50*#3}},{\spherez{#1+0.55*#3}{#2+0.50*#3}}) {};

    %\path[<->] (A) edge[line width=0.3mm] node[ fill=white, anchor=center, pos=0.5] {\large M} (B);
    %\path[<->] (C) edge[line width=0.3mm] node[ fill=white, anchor=center, pos=0.5] {\large M} (D);
  } %>>>
  \drawpatch{\PLat}{\PLon}{70}

\end{tikzpicture} %>>>



==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make verb              #for debugging
##  $ make nobib             #for faster compilation
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler
##
## to have a faster compilation, this does most of passes in quiet
## mode. The downside is that it hides the error in case of
## failure. To see the error either "make verb" or "make VERB='yes'".
###

## user options
VERB	= yes
NOBIB   = no
PROJ    = main #$(notdir $(shell pwd))#defaults to dirname
LXX     = ${PDFLATEX}
OUTEXT  = pdf
SUMMARY = grep "\(error\|warn\|warning\|repeated\|skipping\)" -in --color
SYNC    = -synctex=1
ONEPASS = no
FIGRES  = 300

## programs
PDFLATEX = pdflatex
LATEX	 = latex
BIB	 = bibtex
DVI	 = dvipdf
PS	 = ps2pdf

## internal flag
QUIET	 =
LXFLAG 	 = -file-line-error -halt-on-error -shell-escape ${SYNC}
LXDFLAG  = ${LXFLAG}
BIBEXT   = bbl
INTEXT   = out

ifeq (${VERB},no)
  QUIET = -interaction=batchmode
endif

ifeq (${NOBIB},yes)
  BIBEXT = nobbl
endif

ifeq (${ONEPASS},no)
  LXFDFLAG += -draftmode
else
  INTEXT    = ${BIBEXT}
endif

TEXFILES = $(shell ls *.tex *.bib)

## project rules ##########################################################
###########################################################################
all: $(addsuffix .${OUTEXT}, ${PROJ})

## utility rules ##########################################################
###########################################################################
bib: $(addsuffix .${BIBEXT}, ${PROJ})

help:
	@head -18 ${MAKEFILE_LIST}

verb:   ## verbose make
	${MAKE} VERB=yes all

nobib:
	${MAKE} NOBIB=yes all

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4    	\
	-dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH   	\
	-dDownsampleColorImages=true			 	\
	-dDownsampleGrayImages=true 				\
	-dDownsampleMonoImages=true 				\
        -dColorImageResolution=${FIGRES}			\
        -dGrayImageResolution=${FIGRES}				\
        -dMonoImageResolution=${FIGRES}				\
	-dColorImageDownsampleThreshold=1.5 			\
	-dGrayImageDownsampleThreshold=1.5 			\
	-dMonoImageDownsampleThreshold=1.5 			\
	-sOutputFile=${PROJ}-cmprs.pdf ${PROJ}.pdf

## generic rules ##########################################################
###########################################################################
%.pdf:${TEXFILES}
	${MAKE} LXX=${PDFLATEX} $*.${INTEXT}

%.dvi:${TEXFILES}
	${MAKE} LXX=${LATEX} $*.${INTEXT}

%.out:%.tex ${TEXFILES} %.${BIBEXT}
	${LXX} ${QUIET} ${LXDFLAG} $<
	${LXX} ${QUIET} ${LXFLAG} $<
	${SUMMARY} $*.log $*.blg
#	${MAKE} clean

%.aux:%.tex ${TEXFILES}
	${LXX} ${QUIET} ${LXDFLAG} $<

%.${BIBEXT}:%.aux
	-${BIB} $* 1>/dev/null
	-${SUMMARY} $*.blg

%.nobbl:%.aux
	@echo "skipping the bib make step"

clean:
	${RM} *out *-blx.bib *run.xml *.nav *.snm *.toc *.cb *.cb2 *.spl *.cpt *.tdo *.lof *.lot *.auxlock figs/*.log figs/*.spl *.upa

cleaner:
	${MAKE} clean
	${RM} *log *blg $(addsuffix .aux, ${PROJ}) $(addsuffix .synctex.gz, ${PROJ})
	${RM} figs/*.dpth figs/*.md5 figs/*.dep
cleanest:
	${MAKE} cleaner
	${RM} $(addsuffix .pdf, ${PROJ}) $(addsuffix .dvi, ${PROJ}) $(addsuffix .${OUTEXT}, ${PROJ}) $(addsuffix .bbl, ${PROJ}) figs/tikz-external-* figs/${PROJ}-*

.PHONY: clean cleaner cleanest
.SUFFIXES:
.SECONDARY:

